Real-Time High-Resolution Background Matting

We introduce a real-time, high-resolution background replacement technique which operates at 30fps in 4K resolution, and 60fps for HD on a modern GPU. Our technique is based on background matting, where an additional frame of the background is captured and used in recovering the alpha matte and the foreground layer. The main challenge is to compute a high-quality alpha matte, preserving strand-level hair details, while processing high-resolution images in real-time. To achieve this goal, we employ two neural networks; a base network computes a low-resolution result which is refined by a second network operating at high-resolution on selective patches. We introduce two largescale video and image matting datasets: VideoMatte240K and PhotoMatte13K/85. Our approach yields higher quality results compared to the previous state-of-the-art in background matting, while simultaneously yielding a dramatic boost in both speed and resolution.

==> src/teaser.tex <==
% teaser.tex is referenced in cvpr.cls
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\includegraphics[width=.95\textwidth]{figures/intro_teaser.jpg}
\begin{small}
    \begin{tabularx}{.95\textwidth}{YYY}
        Zoom input and background shot & Zoom with new background & Our Zoom plugin with new background
    \end{tabularx}
\end{small}
\vspace{-0.5em}
\captionof{figure}{
Current video conferencing tools like Zoom can take an input feed (left) and replace the background, often introducing artifacts, as shown in the center result with close-ups of hair and glasses that still have the residual of the original background. Leveraging a frame of video without the subject (far left inset), our method produces real-time, high-resolution background matting without those common artifacts. The image on the right is our result with the corresponding close-ups, screenshot from our Zoom plugin implementation.}
